AutoPrompt: Eliciting Knowledge from Language Models with Automatically Generated Prompts

The remarkable success of pretrained language models has motivated the study of what kinds of knowledge these models learn during pretraining. Reformulating tasks as fill-in-the-blanks problems (e.g., cloze tests) is a natural approach for gauging such knowledge, however, its usage is limited by the manual effort and guesswork required to write suitable prompts. To address this, we develop AutoPrompt, an automated method to create prompts for a diverse set of tasks, based on a gradient-guided search. Using AutoPrompt, we show that masked language models (MLMs) have an inherent capability to perform sentiment analysis and natural language inference without additional parameters or finetuning, sometimes achieving performance on par with recent state-of-the-art supervised models. We also show that our prompts elicit more accurate factual knowledge from MLMs than the manually created prompts on the LAMA benchmark, and that MLMs can be used as relation extractors more effectively than supervised relation extraction models. These results demonstrate that automatically generated prompts are a viable parameter-free alternative to existing probing methods, and as pretrained LMs become more sophisticated and capable, potentially a replacement for finetuning.

==> sections/40-results.tex <==
\section{Sentiment Analysis}
\label{sec:sentiment}

Sentiment analysis is a fundamental task in NLP, both for natural language understanding research and real-world applications.
It is also difficult to probe the extent to which MLMs understand sentiment without finetuning.

\paragraph{Setup}
We apply our method to convert instances from the binary Stanford Sentiment Treebank ~\cite[SST-2]{socher2013recursive} into prompts, using the standard train/test splits.
We find label tokens using a prompt based on the template in Table~\ref{tab:example-templates}.
For our gradient-based prompt search, we perform a grid search over the following hyperparameters: 
$|\mathcal{V}_{cand}| \in \{10, 100\}$, $|\mathcal{V}_{y}| \in \{1, 3, 5\}$, $|\bm{x}_{\textrm{trig}}| \in [3,6]$.\footnote{Required 2 days to run with 8 NVIDIA 2080Ti GPUs.}
All prompts are initialized with the same template used to find the label set.

We also construct a prompt manually (before automated prompts are generated, to avoid bias) 
based on the intuition that SST-2 is comprised of movie reviews. We use
``\prompt{\{sentence\}} \trigger{this movie was} \labtok{[P]}\prompt{.}'' as the template, and use ``{\tt terrible}'' and ``{\tt fantastic}'' for the negative and positive label tokens, respectively.

\begin{table}[tb]
    \small
    \centering
    \begin{tabular}{l cc}
        \toprule
        {\bf Model } & {\bf Dev } & {\bf Test } \\
        \midrule
        BiLSTM & - & $82.8^{\ensuremath{\dagger}}$ \\
        BiLSTM + ELMo & - & $89.3^{\ensuremath{\dagger}}$ \\
        BERT (linear probing) & 85.2 & 83.4 \\
        BERT (finetuned) & - & $93.5^{\ensuremath{\dagger}}$ \\
        RoBERTa (linear probing) & 87.9 & 88.8 \\
        RoBERTa (finetuned) & - & $96.7^{\ensuremath{\dagger}}$ \\
        \midrule
        BERT (manual) & 63.2 & 63.2 \\
        BERT (\methodname) & 80.9 & 82.3 \\
        RoBERTa (manual) & 85.3 & 85.2 \\
        RoBERTa (\methodname) & 91.2 & 91.4 \\
        \bottomrule
    \end{tabular}
    \caption{
    \textbf{Sentiment Analysis}
        performance on the SST-2 test set of supervised classifiers (top) and fill-in-the-blank MLMs (bottom). Scores marked with~\ensuremath{\dagger} are from the GLUE leaderboard: \url{http://gluebenchmark.com/leaderboard}.
    }
    \vskip -5mm
    \label{tab:sst2-test}
\end{table}

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics{figures/sst2_bert_training_size.pdf}
        \caption{BERT on SST-2}
        \label{fig:training:sst2-bert}
    \end{subfigure}
    \qquad
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics{figures/sst2_roberta_training_size.pdf}
        \caption{RoBERTa on SST-2}
        \label{fig:training:sst2-roberta}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics{figures/sicke_bert_training_size.pdf}
        \caption{BERT on SICK-E}
        \label{fig:training:sicke-bert}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics{figures/sicke_roberta_training_size.pdf}
        \caption{RoBERTa on SICK-E}
        \label{fig:training:sicke-roberta}
    \end{subfigure}
    % \vspace{-10pt}
    \caption{
        \textbf{Effect of Training Data} on sentiment analysis and NLI for \methodname vs. finetuning. 
        X-axis is the number of data points used during training.
        Error bars plot the max. and min. accuracies observed over 10 independent runs.
        In the low data regime, \methodname \textit{-*outperforms} finetuning for RoBERTa.
        {\bf NOTE: Finetuning results are erroneous due to a bug. Please see the Errata for corrections. }
    }
    \label{fig:training-size}
\end{figure}


\paragraph{Results}
We show results in Table~\ref{tab:sst2-test}, along with reference scores from the GLUE~\cite{wang2018glue} SST-2 leaderboard, and scores for a linear probe trained over the elementwise average of the LM token representations.
Prompts generated by \methodname reveal that both BERT and RoBERTa have a strong knowledge of sentiment analysis:
without any finetuning, BERT performs comparably to a supervised BiLSTM, and RoBERTa achieves an accuracy on-par with finetuned BERT and ELMo models.
In addition, we observe that our automatically constructed prompts are more effective than manual prompts, and that they are difficult to construct using human intuition: the best template for RoBERTa is 
``{\tt \prompt{\{sentence\}} \trigger{atmosphere alot dialogue Clone totally} \labtok{[P]}\prompt{.}}''
We include results on the effect of the \methodname hyperparameters in Appendix~\ref{sec:sst2-hyper}.

\paragraph{Accuracy in Low-Data Settings}

Although the goal of \methodname is to probe a model's knowledge, we also find that it can achieve high accuracy in the low-data regime. In particular, we measure the development set accuracy of \methodname prompts when using random subsets of 10, 100, and 1000 instances from the training data. We run our prompt search with $|\bm{x}_{\textrm{trig}}|=10$, $|\mathcal{V}_{y}| = 3$, and $|\mathcal{V}_{\textrm{cand}}| = 10$.
We compare to the performance of BERT and RoBERTa finetuned on the same data.
We repeat this experiment 10 times on different randomly sampled sets of data (and seeds for the finetuned models), and display the best-case, worst-case, and average performance in Figure~\ref{fig:training-size}.

We observe that prompts and finetuning perform comparably on average for BERT, however, in the worst-case, finetuning can fail in the low-data regime (consistent with~\citealt{dodge2020fine}).
For RoBERTa, \methodname performs \textit{substantially better} than finetuning when there are 100s to 1000s of training examples.
This excellence in the low-data regime is an interesting phenomenon, and suggests that there is an initial barrier that MLMs must surmount when they are converted to finetuned classifiers that is not encountered when the task is presented as masked language modeling. % format.

\section{Natural Language Inference}
\label{sec:nli}

\begin{table}[tb]
    \small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{\bf Model } & \multicolumn{3}{c}{\bf SICK-E Datasets} \\
        & standard & 3-way & 2-way\\
        \midrule
        Majority  & 56.7 & 33.3  & 50.0\\
        BERT (finetuned)  & 86.7 & 84.0 & 95.6\\
        BERT (linear probing) & 68.0 & 49.5 & 91.9\\
        RoBERTa (linear probing) & 72.6 & 49.4 & 91.1 \\
        \midrule
        BERT (\methodname)   & 62.3 & 55.4 &  85.7\\
        RoBERTa (\methodname)    & 65.0  & 69.3  & 87.3\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Natural Language Inference} performance on the SICK-E test set and variants.
    (Top) Baseline classifiers. (Bottom) Fill-in-the-blank MLMs.
    }
    \label{table:NLI results}
\end{table}

\begin{table*}[tb]
    \small
    \centering
    \begin{tabular}{C{0.40in}L{1.35in}L{1.95in}L{1.9in}}
        \toprule
        {\textbf{Task}} & {\bf Prompt Template} & {\bf Prompt found by \methodname} & {\bf Label Tokens}\\
        \midrule

        %%% ROW %%%
        \multirow{1}{*}{\shortstack[c]{Sentiment\\ Analysis}}
        &   \vspace{-6pt}
            {\tt \prompt{\{sentence\}} \trigger{[T]\ldots[T]}  \labtok{[P]}\prompt{.} } &
            \vspace{-6pt}
            {\tt \prompt{unflinchingly bleak and desperate} \trigger{Writing academicswhere overseas will appear} \labtok{[MASK]}\prompt{.}} &
            \footnotesize{{\bf pos}: partnership, extraordinary, \#\#bla \newline
            {\bf neg}: worse, persisted, unconstitutional}
            \\
        \midrule
        
        %%% ROW %%%
        \multirow{1}{*}{\shortstack[c]{NLI}} & 
            \vspace{-5pt}
            {\tt \prompt{\{prem\}}\labtok{[P]}\trigger{[T]\ldots[T]}\prompt{\{hyp\}}}
        & 
        \vspace{-7pt}
        \tt{\justify{\prompt{Two dogs are wrestling and hugging} \labtok{[MASK]} \trigger{concretepathic workplace} \prompt{There is no dog wrestling and hugging}}}
        & 
        \footnotesize{{\bf con}: Nobody, nobody, nor \newline
        {\bf ent}:  \#\#found, \#\#ways, Agency \newline
        {\bf neu}: \#\#ponents, \#\#lary, \#\#uated }
       \\
        
        %%% ROW %%%
        \midrule
        \multirow{1}{*}{\shortstack[c]{Fact \\ Retrieval}} & 
            {\footnotesize \textit{X plays Y music}} \newline
            {\tt \prompt{\{sub\}}\trigger{[T]\ldots[T]}\labtok{[P]}\prompt{.} }
            &
            \vspace{-7pt}
            {\tt \prompt{Hall Overton}
            {\color{t_magenta} fireplacemade antique son alto} {\color{t_yellow} [MASK]}\prompt{.}} & 
            \\

        %%% ROW %%%
        \midrule
        \multirow{1}{*}{\shortstack[c]{Relation \\ Extraction}} & 
            {\footnotesize \textit{X is a Y by profession}} \newline
            {\tt \prompt{\{sent\}\{sub\}}\trigger{[T]\ldots[T]}\labtok{[P]}\prompt{.}}
            &
            \vspace{-8pt}
            {\tt {\color{t_green} Leonard Wood (born February 4, 1942) is a former Canadian politician.}\newline
            {\color{t_green} Leonard Wood}
            {\color{t_magenta} gymnasium brotherdicative himself another} {\color{t_yellow} [MASK]}\prompt{.}} &
            \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Example Prompts} by \methodname for each task. On the left, we show the prompt template, which combines the input, a number of trigger tokens \trigger{[T]}, and a prediction token \labtok{[P]}. For classification tasks (sentiment analysis and NLI), we make predictions by summing the model's probability for a number of automatically selected label tokens. For fact retrieval and relation extraction, we take the most likely token predicted by the model.}
    \label{tab:example-templates}
\end{table*}

To evaluate the \textit{semantic} understanding of MLMs, we experiment on Natural Language Inference (NLI).
NLI is crucial in many tasks such as reading comprehension and commonsense reasoning~\cite{bowman2015large}, and it is used as a common benchmark for language understanding.

\paragraph{Setup}
We use the entailment task from the SICK dataset~\cite[SICK-E]{marelli2014sick} which consists of around 10,000 pairs of human-annotated sentences labeled as entailment, contradiction, and neutral.
The standard dataset is biased toward the neutral class which represent $56.7$\% of instances.
We also experiment on an unbiased variant with 2-way classification of contradiction vs. entailment (\textit{2-way}), as well as an unbiased 3-way classification variant (\textit{3-way}). 
The template used for \methodname is provided in Table~\ref{tab:example-templates}.
We search over the following parameters: $|\mathcal{V}_{cand}| \in \{10, 50\}$, $|\mathcal{V}_{y}| \in \{1, 3, 5, 10\}$, $|\bm{x}_{\textrm{trig}}| \in [1,5]$, and choose the best prompt according to development set accuracy.

\paragraph{Results}
Table~\ref{table:NLI results} shows that \methodname considerably outperforms the majority baseline in all experiments.
For example, on the 2-way SICK-E dataset, \methodname is comparable to a supervised finetuned BERT.
We also test linear probes---linear classifiers trained on top of frozen MLM representations with average pooling ---and find \methodname has comparable or higher accuracy, despite linear probes being susceptible to false positives. 
Overall, these results demonstrate that both BERT and RoBERTa have some inherent knowledge of natural language inference.

We also examine the efficacy of \methodname in the low-data regime (using the same procedure as SST-2) on the unbiased 3-way SICK-E data. The results in Figure~\ref{fig:training-size} show that \methodname performs on par with finetuned BERT and significantly better than finetuned RoBERTa in low data settings. 




\paragraph{MLMs Excel on Contradiction}
We find that the label tokens are more interpretable for \emph{contradiction} compared to \textit{entailment} or \textit{neutral} (examples in Table~\ref{tab:example-templates}).
We investigate if this hurts the model performance on entailment and neutral classes. 
We measure the precision for each label in the 3-way balanced SICK-E dataset.
BERT achieves $74.9$\%, $54.4$\%, and $36.8$\% precision for contradiction, entailment, and neutral cases, respectively, while RoBERTa obtains $84.9$\%, $65.1$\%, and $57.3$\%. %, respectively.
These results suggest that \methodname may be more accurate for concepts that can be easily expressed using natural label tokens. % (e.g., contradiction).



\section{Fact Retrieval}
\label{sec:factual}

An important question is whether pretrained MLMs \emph{know} facts about real-world entities.
The LAMA dataset~\cite{petroni2019language} evaluates this using cloze tests that consist of \texttt{(sub, rel, obj)} triples, e.g. (\texttt{Obama}, \texttt{bornIn}, \texttt{Hawaii}), and \textit{manually} created prompts with missing objects, e.g. ``\prompt{Obama} \trigger{was born in} \labtok{[MASK]}\prompt{.}''.
LPAQA~\cite{jiang2019can} extends this idea by \textit{systematically} creating prompts that are generated by mining Wikipedia, paraphrasing, and crowdsourcing. 
In this section, we use the same cloze-style setup but \emph{automatically} generate prompts in order to better evaluate the factual knowledge of MLMs. We compare our approach against LAMA and LPAQA, which are explicitly designed for the task of fact retrieval.

\paragraph{Setup}
We reformulate fact retrieval by mapping \texttt{(sub,rel,obj)} triples to a prompt using the template ``\prompt{\{sub\}}\trigger{[T]\ldots[T]}\labtok{[P]}\prompt{.}'', where the trigger tokens are specific to the relation \texttt{rel} and the correct object \texttt{obj} is the label token.
We use the original test set from LAMA~\cite{petroni2019language}, henceforth \emph{Original}. To collect training data for \methodname, we gather at most 1000 facts for each of the 41 relations in LAMA from the T-REx dataset~\cite{DBLP:conf/lrec/ElSaharVRGHLS18}. For the relations that still have less than 1000 samples, we gather extra facts straight from Wikidata. We ensure that none of the T-REx triples are present in the test set, and we split the data 80-20 into train and development sets. Moreover, because the collected T-REx data is from a slightly different distribution than the LAMA test set, we also consider a separate evaluation where we split the T-REx triples into a 60-20-20 train/dev/test split and evaluate on the test set. This \emph{T-REx} dataset is used to measure the performance of our prompts when the train and test data is from the same distribution.

We use \methodname with 5 or 7 tokens, and select the search parameters using the T-REx development set.
We prevent proper nouns and tokens that appear as gold objects in the training data from being selected as trigger tokens. 
This is done to prevent \methodname from ``cheating'' by embedding common answers inside the prompt.
To evaluate, we observe the rank of the true object in label token distribution of the MLM, and use standard ranking metrics: mean reciprocal rank (MRR), precision-at-1 (P@1), and precision-at-10 (P@10).

\begin{table*}[tb]
\begin{subtable}{.55\linewidth}
    \small
    \centering
    \begin{tabular}{lrrrrrr}
    \toprule
    \multirow{3}{*}{\bf Prompt Type} & \multicolumn{3}{c}{\bf Original} & \multicolumn{3}{c}{\bf T-REx} \\
    
     \cmidrule(lr){2-4}
     \cmidrule(lr){5-7}
     & MRR & P@10 & P@1  & MRR & P@10 & P@1 \\
    \midrule
    LAMA & 40.27 & 59.49 & 31.10 & 35.79 & 54.29 & 26.38 \\
    LPAQA (Top1) & 43.57 & 62.03 & 34.10 & 39.86 & 57.27 & 31.16 \\
    \methodname 5 Tokens & 53.06 & 72.17 & 42.94 & 54.42 & 70.80 & 45.40 \\
    \methodname 7 Tokens & 53.89 & 73.93 & 43.34 & 54.89 & 72.02 & 45.57 \\
    \bottomrule
    \end{tabular}
\end{subtable}%
\hspace{.12\linewidth}%
\begin{subtable}{.30\linewidth}
    \small
    \centering
    \begin{tabular}{lccc}
    \toprule
    \bf Model & MRR & P@10 & P@1 \\
    \midrule
    BERT & 55.22 & 74.01 & 45.23 \\
    RoBERTa & 49.90 & 68.34 & 40.01 \\
    \bottomrule
    \end{tabular}
    \end{subtable}
    \caption{\textbf{Factual Retrieval: } On the left, we evaluate BERT on fact retrieval using the \emph{Original} LAMA dataset from \citet{petroni2019language}. For all three metrics (mean reciprocal rank, mean precision-at-10 (P@10), and mean precision-at-1(P@1)), \methodname significantly outperforms past prompting methods. We also report results on a \emph{T-REx} version of the data (see text for details). On the right, we compare BERT versus RoBERTa on a subset of the LAMA data using \methodname with 5 tokens.
    }
\label{tab:fact-ret}
\end{table*}


\paragraph{Results}
Table~\ref{tab:fact-ret} shows the performance of MLMs with different prompting methods, and we show qualitative examples in Table~\ref{tab:example-templates} and in Appendix~\ref{app:factual}.
Prompts generated using \methodname can extract factual knowledge from BERT more effectively than their manual and mined counterparts: we improve P@1 by up to 12 points.
Moreover, despite \methodname using only one prompt per relation, it still outperforms LPAQA's ensemble method (which averages predictions for up to 30 prompts) by approximately 4 points.
Using 7 trigger tokens achieves slightly higher scores than 5 trigger tokens, although the difference is not substantial. This indicates that our approach is stable to the choice of trigger length, which is consistent with our sentiment analysis results.
Overall, these results show that \methodname can retrieve facts more effectively than past prompting methods, thus demonstrating that \bert contains more factual knowledge than previously estimated.

\paragraph{Relation Breakdown}
We also provide a detailed breakdown of the prompts found by \citet{petroni2019language} and \methodname, and their associated accuracies in Appendix~\ref{app:factual}, Table~\ref{tab:fact-ret-rob}. 
Manual prompts are competitive when the prompt is \textit{easy} to specify, e.g., the prompt \emph{``was born in''} for the \textsc{place of birth} relation.
On the other hand, \methodname performs especially well for relations that are difficult to specify in a natural language prompt.
For example, \citet{petroni2019language}'s prompt for the \textsc{position played on team} relation is ``\prompt{\{sub\}} \trigger{plays in} \labtok{[MASK]} \trigger{position}'', which is not as specific as the relation requires.
Although the prompt from \methodname is not grammatical (\emph{``\prompt{\{sub\}} \trigger{ediatric striker ice baseman defensive} \labtok{\{obj\}}''}), it does contain tokens that are directly related to sports.

\paragraph{BERT outperforms \roberta} We finally directly compare BERT and RoBERTa. To do so, we subsample the LAMA test set to consist of examples where the object is a single token for both BERT and RoBERTa (\textit{Original-RoBERTa}).\footnote{The original dataset consists of examples where the object is a single token for BERT.}
\bert actually slightly outperforms RoBERTa, and we find that the prompts generated for RoBERTa tend to contain more irrelevant words (see Appendix~\ref{app:factual}, Table~\ref{tab:fact-ret-rob}).
For example, the prompt generated by RoBERTa for the \textsc{plays instrument} relation contains words such as ``Trump'' and symbols such as ``,'' (),'' for the \textsc{position played on team} relation. 
It is surprising that \roberta does not perform better than \bert, and it is worthy of investigating this further in future work.
Additionally, recall that prompting is a \emph{lower bound} on a model's knowledge: the lower relative performance does not mean that the model actually knows less.

\section{Relation Extraction}
\label{sec:ie}

Apart from evaluating whether MLMs \emph{know} facts, it is also important to evaluate whether they can \emph{extract knowledge} from text.
In this section, we use the task of relation extraction (RE)---to identify how entities are related in a given sentence---an important task in information extraction.
We create RE prompts in a similar fashion as fact retrieval: for a given triple \texttt{(subj,rel,obj)} and sentence that expresses this relation, we construct a prompt as ``\prompt{\{sent\}\{sub\}}\trigger{[T]\ldots[T]}\labtok{[P]}\prompt{.}'', where the trigger tokens are specific to the relation, and label token is the correct object \texttt{obj} (see Table~\ref{tab:example-templates} for an example).

\paragraph{Setup}
We use the T-Rex dataset for RE because each T-REx fact comes with context sentences that mention the subject and object surface forms.
We compare \methodname to LAMA and LPAQA (their prompts are still useful here), as well as a recent supervised relation extraction model~\cite{DBLP:conf/emnlp/SorokinG17} that was also used by \citet{petroni2019language}. To make the evaluation fair for the supervised RE model, we modify the standard RE evaluation. We give the model credit as long as it does not predict a different relation for the subject and object, i.e. we ignore the ``no relation'' prediction and all other relations. We also drop all sentences from evaluation for which the model's named entity extractor failed to identify the subject and the object as entities.
See Appendix~\ref{app:re} for further details. For the evaluation of all systems, we treat a prediction as correct if it is either the canonical version of the object (e.g., ``USA'') or the rendered surface form (e.g., ``American'') for \textit{any} of the context sentences in a given triple.

\paragraph{Results}
Table~\ref{tab:RE} shows the results for BERT and RoBERTa. 
MLMs can extract relational information \textit{more effectively} than the supervised RE model,
providing up to a 33\% increase on the task when using \methodname.
RoBERTa also outperforms the supervised RE model, although it is worse than BERT (likely for similar reasons as we outline in Section~\ref{sec:factual}).
For both BERT and RoBERTa, we notice that the trigger tokens consist of words related to their corresponding relations (see Appendix~\ref{app:rel}, Table~\ref{tab:RE-examples} for full list), e.g. RoBERTa selects {\trigger{``defy trademarks of namesake manufacturer''}} for relation \textsc{manufacturer/producer of product}.

\paragraph{Perturbed Sentence Evaluation}
A possible explanation for the strong results of MLMs in the RE setting is that they may \textit{already} know many of the relations. Thus, they may directly predict the objects instead of \textit{extracting} them.
To separate this effect, we synthetically perturb the relation extraction dataset by replacing each object in the test data with a random other object and making the same change to the prompt. For example, \emph{``Ryo Kase (born November 9, 1974 in \st{Yokohama}$\rightarrow$Yorkshire) is a Japanese actor''} where \texttt{Ryo Kase} is the subject, \texttt{Yokohama} is the original object, and \texttt{Yorkshire} is the new object.
We regenerate the prompts using the perturbed version of the data.

The accuracy of the RE model does not change significantly on the perturbed data (Table~\ref{tab:RE}), however, the accuracy of the MLMs decreases significantly.
This indicates that a significant portion of MLM accuracy comes from background information rather than relation extraction.
Nevertheless, our prompts for BERT outperform their LAMA and LPAQA counterparts, which provides further evidence that \methodname produces better probes.

\begin{table}[tb]
\small
    \centering
    \begin{tabular}{lrr}
    \toprule
    \bf Model & \bf Original & \bf Perturbed \\
    \midrule
    Supervised RE LSTM & 57.95 & 58.81\\
    BERT (LAMA) & 69.06 & 28.02 \\
    BERT (LPAQA) & 76.55 & 30.79 \\
    BERT (\methodname) & 90.73 & 56.43 \\
    RoBERTa (\methodname) & 60.33 & 28.95 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Relation Extraction:} We use prompts to test pretrained MLMs on relation extraction. Compared to a state-of-the-art LSTM model from 2017, MLMs have higher mean precision-at-1 (P@1), especially when using prompts from \methodname. We also test models on sentences that have been edited to contain incorrect facts. The accuracy of MLMs drops significantly on these sentences, indicating that their high performance stems from their factual knowledge.}
    \label{tab:RE}
\end{table}

==> sections/intro-v2.tex <==
\section{Abstract}

Pretrained language models (LMs) have had exceptional success when adapted to downstream tasks via \emph{finetuning}~\cite{PetersELMo2018, devlin2018BERT}.
% Although it is clear that knowledge learned during pretraining transfers to downstream tasks, we have little understanding of how much knowledge the pretrained models contain.
% In particular, it is unclear how much task-specific information is added to the pretrained model during finetuning, as opposed to knowledge attained during the language model pretraining itself.
Although it is clear that pretraining improves accuracy, it is difficult to determine whether the knowledge that finetuned LMs contain is learned during the \textit{pretraining} or the \textit{finetuning} process.
How can we directly evaluate the knowledge present in pretrained LMs, be it linguistic, factual, commonsense, or task-specific?

Numerous techniques have been proposed to elicit such knowledge by analyzing pretrained LMs' internal representations.
A common strategy is to use probing classifiers---shallow classifiers that predict certain attributes using an LMs' representations as features~\cite{conneau2018you,liu2019linguistic}.
However, probing classifiers require additional learned parameters and are thus susceptible to false positives; high probing accuracy is \textit{not} a sufficient condition to conclude that an LM contains a certain piece of knowledge~\cite{hewitt2019designing,voita2020information}.
Attention visualization, another common technique, has a similar failure mode: attention scores may be correlated with, but not caused by the underlying target knowledge, leading to criticism against their use as explanations~\cite{jain2019attention,wiegreffe2019attention}. Both probing and attention visualizations also struggle to evaluate knowledge that cannot be represented as simple token- or sequence-level classification tasks.

\begin{figure*}[tb]
    \centering
    \includegraphics{figures/hook_figure_two_col.pdf}
    \caption{
        {\bf Illustration of \methodname} applied
        to probe a masked language model's (MLM's) ability to perform sentiment analysis.
        Each input, $\bm{x}_{\textrm{inp}}$, is placed into a natural language prompt, $\bm{x}_{\textrm{prompt}}$, which contains a single {\tt[MASK]} token.
        The prompt is created using a template, $\lambda$, which combines the original input with a set of trigger tokens, $\bm{x}_{\textrm{trig}}$.
        The trigger tokens are shared across all inputs and determined using a gradient-based search).
        Probabilities for each class label, $y$, are then obtained by marginalizing the MLM predictions, $p(\textrm{\tt[MASK]}|\bm{x}_{\textrm{prompt}})$, over sets of automatically detected label tokens).
    }
    \label{fig:hook}
\end{figure*}

A more direct approach for eliciting knowledge from these models, since they are language models after all, is \emph{prompting}, i.e. converting tasks into a language model format.
For example, \citet{radford2019gpt2} frame summarization as a language modeling task by appending ``TL;DR:'' to the end of an article and then generating from an LM.
Similarly, \citet{petroni2019language} manually reformulate a knowledge base completion task as a cloze test (i.e., a fill-in-the-blank problem).
Compared to existing model analysis methods, prompting is non-invasive: it does not introduce large amounts of additional parameters or require direct inspection of a model's representations.
Thus prompting provides a lower bound on what the model ``knows'', and is therefore a more useful analysis tool.
However, prompting unfortunately requires manually crafting the context to feed into the model.
Not only is this time consuming and non-intuitive for many tasks (e.g., textual entailment), more importantly, models are highly sensitive to this context: improperly-constructed contexts cause artificially low performance~\cite{jiang2019can}. 
Overcoming the need to manually specify prompts would make prompting a more widely useful analysis tool.

In this paper, we introduce \methodname---an \emph{automated} method for generating prompts for any task,
illustrated in Figure~\ref{fig:hook}.
Given a task, e.g., sentiment analysis, \methodname creates a prompt by combining the original task inputs (e.g. reviews) with a collection of \emph{trigger tokens} according to a template.
The same set of trigger tokens is used for all inputs, and is learned using a variant of the gradient-based search strategy proposed in \citet{Wallace2019Triggers}.
The LM predictions for the prompt are converted to class probabilities by marginalizing over a set of associated label tokens, which can either be learned or specified ahead of time, enabling the LM to be evaluated the same as one would any other classifier.

We validate the effectiveness of \methodname in numerous experiments.
First, we use \methodname to construct prompts that test pretrained masked language models (MLMs) on sentiment analysis and natural language inference (NLI).
Our tests reveal that, without any finetuning, MLMs perform well on both of these tasks---a properly-prompted \roberta achieves 91\% accuracy on SST-2 (better than a finetuned ELMo model~\cite{PetersELMo2018}), and 69\% accuracy
on a balanced variant of the SICK-E dataset \cite{marelli2014sick}.
Next, we apply \methodname to the fact retrieval tasks of LAMA~\cite{petroni2019language}, where we are able to construct prompts that more effectively elicit MLM's factual knowledge than existing prompts generated using manual and corpus-mining methods.
Concretely, we achieve 43.3\% precision-at-1, compared to the current best single-prompt result of 34.1\%~\cite{jiang2019can}.
We also introduce a variant of this task, similar to relation extraction (RE), that tests whether MLMs can extract knowledge from a given piece of text.
We show that MLMs can actually \emph{outperform} existing RE models when context sentences with real facts are provided, however, they struggle when context sentences are artificially falsified.

Finally, although the goal of \methodname is to analyze models, we find that it provides certain practical advantages over finetuning. First, \methodname achieves higher average- and worst-case accuracy than finetuning in low-data regimes. Moreover, unlike finetuning, prompting LMs does not require large amounts of disk space to store model checkpoints; once a prompt is found, it can be used on off-the-shelf pretrained LMs. This is beneficial when serving models for multiple tasks.
